MAP-Music2Vec: A Simple and Effective Baseline for Self-Supervised Music Audio Representation Learning

The deep learning community has witnessed an exponentially growing interest in self-supervised learning (SSL). However, it still remains unexplored how to build a framework for learning useful representations of raw music waveforms in a self-supervised manner. In this work, we design Music2Vec, a framework exploring different SSL algorithmic components and tricks for music audio recordings. Our model achieves comparable results to the state-of-the-art (SOTA) music SSL model Jukebox, despite being significantly smaller with less than 2% of parameters of the latter. The model will be released on Huggingface(Please refer to: https://huggingface.co/m-a-p/music2vec-v1)

==> macro.tex <==
\newcommand{\todo}[1]{{\color{blue} TODO: {#1}}}
% changed to magenta because there was an error about purple
\newcommand{\rc}[1]{{\color{magenta}{[RC: #1]}}}
\newcommand{\cd}[1]{{\color{blue}{[CD: #1]}}}
\newcommand{\pl}[1]{\textcolor{red}{[PL: #1]}}
%\newcommand{\pl}[1]{{\color{red} [P] {#1}}}


\newcommand{\gtzanacc}{GTZAN}
\newcommand{\mttauc}{$\text{MTT}_{\text{AUC}}$}
\newcommand{\mttap}{$\text{MTT}_{\text{AP}}$}
\newcommand{\emoa}{$\text{Emo}_{\text{A}}$}
\newcommand{\emov}{$\text{Emo}_{\text{V}}$}
\newcommand{\gssco}{GS}
\newcommand{\gmueavg}{Average}

\newcommand{\rsquared}{$R^2$}

\newcommand{\calm}{CALM}

\newcommand{\rep}[1]{\textsc{#1}}
\newcommand{\repmfcc}{\rep{MFCC}}
\newcommand{\repchroma}{\rep{Chroma}}
\newcommand{\repclmr}{\rep{CLMR}}
\newcommand{\repchoi}{\rep{Choi}}
\newcommand{\repmusicnn}{\rep{MusiCNN}}
\newcommand{\repjuke}{\rep{Jukebox}}

\newcommand{\etal}{et~al.}

==> table.tex <==
%Please add the following packages if necessary:
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[tbh]\centering
\caption{
Preliminary Results on MIR Tasks. The baseline results and probing protocol are adopted from JukeMIR~\cite{castellon2021codified}. All results are produced with {probing\textsuperscript{$\diamondsuit$}} or {fine-tuning\textsuperscript{$\spadesuit$}} settings.
}
\label{tab:preliminary_mir}
% \scriptsize
\scalebox{0.75}{
\begin{tabular}{lrrrrr}\toprule
\textbf{Task} &\multicolumn{2}{c}{\textbf{Auto Tagging}} &\textbf{Genre} &\textbf{Key} \\
\cmidrule{1-5}
\textbf{Model} &\textbf{MTT}{\tiny AUC}\uparrow &\textbf{MTT}{\tiny MAP}\uparrow &\textbf{GTZAN}{\tiny ACC}\uparrow &\textbf{GS}{\tiny Score}\uparrow \\\midrule
CHOI\textsuperscript{$\diamondsuit$} &89.7 &36.4 &75.9 & 13.1 \\
CLMR\textsuperscript{$\diamondsuit$} &89.4 &36.1 &68.6 & 14.9 \\
MusiCNN\textsuperscript{$\diamondsuit$} &90.6 &38.3 & 79.0 & 12.8 \\
Jukebox\textsuperscript{$\diamondsuit$} (5B) &91.5 &41.4 & 79.7 & 66.7 \\
\midrule
Ours-base\textsuperscript{$\diamondsuit$} (90M) & (90.8) & (38.4) & (80.7) & (67.0) \\
Ours-base\textsuperscript{$\spadesuit$} (90M) & - & - & - & (69.5) \\
% \hline
\bottomrule
\end{tabular}
}
\end{table}



